Anticipate and Learn: Unleashing Idle-Time Compute in Proactive Agents

While AI agents demonstrate remarkable capabilities in reasoning and tool use, they remain fundamentally reactive: they compute responses only after explicit user prompts. This paradigm ignores a critical opportunity: the idle time between interactions is largely wasted, leaving agents unable to prepare for future user needs. To bridge this gap, we introduce ProAct, a proactive agent architecture that leverages idle-time compute to anticipate and fulfill likely upcoming user needs. By analyzing evolving dialogue history together with persistent memory, ProAct predicts upcoming needs and iteratively acquires information, allowing the agent to resolve knowledge gaps and prepare evidence before the user initiates a query. To rigorously evaluate proactive capabilities, we also introduce ProActEval, a comprehensive benchmark comprising 200 scenarios across 40 domains, featuring predictable need chains and diverse user cognitive profiles. Empirical results demonstrate significant advantages over reactive baselines. ProAct accelerates task completion by reducing required turns by 14.8%, decreases user effort by 11.7%, and cuts hallucination rates by 28.1% on ProActEval. Furthermore, MemBench evaluations confirm that ProAct achieves state-of-the-art reflective accuracy, underscoring its sustained and robust performance.

==> sections/abstract.tex <==
\begin{abstract}
% LLM-based conversational agents are increasingly capable at reasoning, tool use, and multi-turn response generation, but most still operate reactively, responding only after a user asks.
% This pattern leaves two gaps: agents rarely predict future information needs, and the idle time between interactions is left unused even when it could support later turns.
% We present \system{}, a proactive assistant architecture that predicts likely upcoming user needs from the evolving dialogue and persistent user context, then uses idle periods for value-aware search, synthesis, and delivery before those needs are explicitly requested.
% A personalized memory system supports both modules by grounding predictions, tracking knowledge gaps, and storing newly acquired information.
% We also introduce ProActEval, a 200-scenario, 40-domain benchmark for closed-world evaluation of proactive assistance with fact sheets, predictable need chains, and five cognitive archetypes.
% On ProActEval, \system{} reduces turns to complete must-have coverage by 14.8\%, reduces user effort by 11.7\%, increases total coverage by 7.2\%, and reduces hallucination rate by 28.1\% over a reactive baseline.
% On MemBench, \system{} reaches 84.3\% reflective accuracy at 10k tokens and 86.3\% at 100k tokens, showing that the supporting memory layer remains effective as context length increases.

While AI agents demonstrate remarkable capabilities in reasoning and tool use, they remain fundamentally reactive: they compute responses only after explicit user prompts. This paradigm ignores a critical opportunity: the \textit{idle time} between interactions is largely wasted, leaving agents unable to prepare for future user needs. To bridge this gap, we introduce \system, a proactive agent architecture that leverages idle-time compute to anticipate and fulfill likely upcoming user needs. By analyzing evolving dialogue history together with persistent memory, \system predicts upcoming needs and iteratively acquires information, allowing the agent to resolve knowledge gaps and prepare evidence before the user initiates a query.  
To rigorously evaluate proactive capabilities, we also introduce \benchmark, a comprehensive benchmark comprising 200 scenarios across 40 domains, featuring predictable need chains and diverse user cognitive profiles. Empirical results demonstrate significant advantages over reactive baselines. \system accelerates task completion by reducing required turns by 14.8\%, decreases user effort by 11.7\%, and cuts hallucination rates by 28.1\% on \benchmark. Furthermore, MemBench evaluations confirm that \system achieves state-of-the-art reflective accuracy, underscoring its sustained and robust performance.
\end{abstract}


==> sections/experiments.tex <==
% ====================================================================
% Section 5: Experiments
% ====================================================================

\section{Experiments}
\label{sec:experiments}

% We evaluate \system{} on two benchmarks.
% MemBench measures whether the supporting memory layer can preserve reflective user information over long contexts.
% ProActEval measures whether idle-time proactive behavior reduces user effort, improves coverage, and preserves factual grounding.

We organize the evaluation around two main questions.
(1) We ask whether prediction-guided idle-time compute improves proactive assistance in multi-turn conversations.
We answer this question on \textbf{ProActEval}, where each scenario provides a fact sheet and an ordered sequence of user needs.
We compare three conditions: a reactive assistant, an undirected Idle-Time compute variant, and the full prediction-guided system.
This comparison evaluates the end-to-end benefit of proactive assistance while also ablating predictive direction: the gap between Undirected Idle and the full system tests whether background search alone is sufficient, or whether idle-time compute must be assigned to predicted needs. 
(2) We ask whether the memory backbone can reliably support such proactive behavior by preserving long-horizon user information.
We answer this question on \textbf{MemBench}, focusing on its reflective participation setting, which tests whether a system can infer user preferences and emotions from accumulated interaction history.
Finally, we extend the analysis by varying the idle-search budget on ProActEval to study the cost--efficiency trade-off of proactive computation.

\begin{table*}[t]
\caption{Main end-to-end results across MemBench and ProActEval. MemBench reports reflective accuracy. ProActEval reports interaction-level efficiency, coverage, and factual-integrity endpoints; metrics are dataset-native and should not be averaged across benchmarks.}
\label{tab:overall-main}
\centering
\small
\begin{tabular}{@{}l cc@{}}
\toprule
\multicolumn{3}{l}{\textbf{(a) MemBench: reflective memory}} \\
\textbf{Method} & \textbf{10k Acc.} $\uparrow$ & \textbf{100k Acc.} $\uparrow$ \\
\midrule
Best prior baseline & 0.742 & 0.833 \\
\system{}           & \textbf{0.843} & \textbf{0.863} \\
\bottomrule
\end{tabular}

\vspace{0.6em}

\begin{tabular}{@{}l c c c c@{}}
\toprule
\multicolumn{5}{l}{\textbf{(b) ProActEval: proactive assistance}} \\
\textbf{Condition} & \textbf{$T_{100}$} $\downarrow$ & \textbf{User Effort} $\downarrow$ & \textbf{Total Cov.} $\uparrow$ & \textbf{Hallucination} $\downarrow$ \\
\midrule
Reactive       & 8.110 & 9.140 & 0.892 & 0.132 \\
Undirected Idle & 8.040 & 9.040 & 0.905 & 0.124 \\
Directed Idle  & \textbf{6.910} & \textbf{8.075} & \textbf{0.956} & \textbf{0.095} \\
\bottomrule
\end{tabular}
\end{table*}


% \subsection{Benchmarks and Evaluation Targets}
% \paragraph{MemBench.}
% MemBench \citep{tan2025membench} evaluates LLM-based memory systems across factual and reflective tasks under participation and observation settings.
% We focus on the reflective participation setting because it tests whether a system can infer preferences and emotions from accumulated interaction history.
% This capability is important for proactive agents because prediction quality depends on persistent user context.
% \paragraph{ProActEval.}
% ProActEval evaluates proactive assistance in closed-world multi-turn conversations.
%Each scenario contains a fact sheet and an ordered sequence of user needs.
% The main outcome is not only whether the assistant is factually correct, but whether it can cover future-relevant needs before the user asks.
% We therefore report efficiency, coverage, anticipation, factual-integrity, and compute-cost metrics.

% \subsection{Main End-to-End Results}

% Table~\ref{tab:overall-main} summarizes the main end-to-end results on the two benchmarks using each benchmark's native primary endpoints.
% On MemBench, \system{} outperforms published structured-memory baselines at both context lengths.
% On ProActEval, the full proactive system improves interaction efficiency, coverage, and factual integrity; Fact Accuracy is reported in the detailed ProActEval table below.

\subsection{Main Proactivity Evaluation}

We evaluate proactive assistance on all 200 ProActEval scenarios by comparing a reactive baseline, an Idle-Time Acquisition variant without predictive direction, and the full prediction-guided \system{}.
\textsc{Reactive} is a non-proactive baseline that disables both \textsc{Future-State Prediction} and \textsc{Idle-Time Acquisition}.
\textsc{Undirected Idle} enables \textsc{Idle-Time Acquisition} but removes predictive direction, using unguided background intents.
\textsc{Directed Idle} is the full \system{} configuration, enabling both \textsc{Future-State Prediction} and \textsc{Idle-Time Acquisition}.
This design allows us to measure the end-to-end benefit of proactive assistance while isolating the contribution of predictive direction.

\paragraph{Overall Proactive Gains.}
Table~\ref{tab:proacteval-main} shows that \textsc{Directed Idle} improves every non-cost metric over both \textsc{Reactive} and \textsc{Undirected Idle}.
Compared with \textsc{Reactive}, it reduces $T_{80}$ by 16.4\%, $T_{100}$ by 14.8\%, and User Effort by 11.7\%, while increasing Total Coverage from 0.892 to 0.956 and Must-Have Coverage from 0.938 to 0.977.
It also improves factual integrity, increasing Fact Accuracy from 0.972 to 0.985 and reducing Hallucination Rate from 0.132 to 0.095.
These results indicate that prediction-guided proactive computation can improve interaction efficiency and coverage while preserving factual grounding.

\begin{table*}[t]
\caption{ProActEval results over 200 scenarios. Arrows indicate the preferred direction. Delta columns report signed percentage changes for Directed Idle relative to each baseline, except Anticipation Recall and Active Tokens, where deltas are absolute. Active Tokens are measured in additional active-token cost.}
\label{tab:proacteval-main}
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l c c c c c@{}}
\toprule
\textbf{Metric} & \textbf{Reactive} & \textbf{Undirected Idle} & \textbf{Directed Idle} & \textbf{$\Delta$ vs. Reactive} & \textbf{$\Delta$ vs. Undirected} \\
\midrule
\multicolumn{6}{l}{\textbf{Efficiency}} \\
\quad $T_{80}$ $\downarrow$              & 6.615 & 6.600 & \textbf{5.530} & $-16.4\%$ & $-16.2\%$ \\
\quad $T_{100}$ $\downarrow$             & 8.110 & 8.040 & \textbf{6.910} & $-14.8\%$ & $-14.1\%$ \\
\quad User Effort $\downarrow$           & 9.140 & 9.040 & \textbf{8.075} & $-11.7\%$ & $-10.7\%$ \\
\midrule
\multicolumn{6}{l}{\textbf{Coverage and Anticipation}} \\
\quad Total Coverage $\uparrow$          & 0.892 & 0.905 & \textbf{0.956} & $+7.2\%$ & $+5.6\%$ \\
\quad Must-Have Coverage $\uparrow$      & 0.938 & 0.950 & \textbf{0.977} & $+4.2\%$ & $+2.9\%$ \\
\quad Anticipation Recall $\uparrow$     & 0.000 & 0.000 & \textbf{0.428} & $+0.428$ & $+0.428$ \\
\midrule
\multicolumn{6}{l}{\textbf{Factual Integrity and Cost}} \\
\quad Fact Accuracy $\uparrow$           & 0.972 & 0.972 & \textbf{0.985} & $+1.3\%$ & $+1.3\%$ \\
\quad Hallucination Rate $\downarrow$    & 0.132 & 0.124 & \textbf{0.095} & $-28.1\%$ & $-23.1\%$ \\
\quad Active Tokens $\downarrow$         & \textbf{0}     & 69.8k & 111.8k & +111.8k & +42.0k \\
\bottomrule
\end{tabular}}
\end{table*}


\paragraph{Ablation Study.}
The comparison between \textsc{Undirected Idle} and \textsc{Directed Idle} isolates the value of predictive direction.
Although \textsc{Undirected Idle} performs Idle-Time Acquisition and spends 69.8k active tokens per scenario on average, it only slightly improves over \textsc{Reactive}, reducing $T_{100}$ by 0.9\% and User Effort by 1.1\%.
By contrast, adding predictive direction in \textsc{Directed Idle} reduces $T_{100}$ by 14.1\% and User Effort by 10.7\% relative to \textsc{Undirected Idle}, and achieves an Anticipation Recall of 0.428 where both other settings remain at 0.
These results suggest that the gains do not come from Idle-Time acquisition alone, but from directing that acquisition toward predicted needs.

\paragraph{Comparison with ProactiveAgent.}
We adapt the public ProactiveAgent decision protocol~\citep{lu2024proactive} as a GPT-4o prompting baseline. Since this baseline sees the user profile and full fact sheet but does not expose structured delivered fact IDs, we compare systems using judge-labeled Anticipation Recall rather than runtime fact-ID matching.

\begin{table*}[t]
\caption{Comparison with ProactiveAgent on 200 ProActEval scenarios. Judge-labeled Ant.R. is the scenario-level macro average; Anticipated Needs reports the corresponding micro count over all predictable needs.}
\label{tab:proactiveagent-comparison}
\centering
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l c c c c c@{}}
\toprule
\textbf{Method} & \textbf{$T_{80}$} $\downarrow$ & \textbf{$T_{100}$} $\downarrow$ & \textbf{User Effort} $\downarrow$ & \textbf{Judge-labeled Ant.R.} $\uparrow$ & \textbf{Anticipated Needs} $\uparrow$ \\
\midrule
\textsc{ProactiveAgent} & 5.600 & 7.145 & 8.425 & 0.020 & 32 / 1,572 \\
\system{} (\textsc{Directed Idle}) & \textbf{5.530} & \textbf{6.910} & \textbf{8.075} & \textbf{0.447} & \textbf{703 / 1,572} \\
\bottomrule
\end{tabular}}
\end{table*}

Table~\ref{tab:proactiveagent-comparison} shows that ProactiveAgent's proactive behavior remains largely turn-local: it anticipates only 32 of 1,572 predictable needs, yielding 0.020 judge-labeled Anticipation Recall.
By contrast, \system{} anticipates 703 of 1,572 predictable needs, reaching 0.447 judge-labeled Anticipation Recall while also modestly improving turn efficiency over ProactiveAgent.


\subsection{Memory Evaluation}
\label{sec:exp:membench}


We evaluate whether the memory backbone can support proactive assistance by preserving long-horizon user information.
We use the reflective participation setting of MemBench at 10k and 100k token scales with Qwen2.5-7B-Instruct.
The main metric is reflective accuracy, which measures whether the system can infer user preferences and emotions from accumulated interaction history.
We compare against FullMemory, RecentMemory, RetrievalMemory, GenerativeAgent~\citep{park2023generative}, MemoryBank~\citep{zhong2024memorybank}, MemGPT~\citep{packer2023memgpt}, and SCMemory~\citep{wang2023enhancing}.


\begin{table}[t]
\caption{Overall reflective accuracy on MemBench. Baseline numbers are aggregate reflective accuracy from the published MemBench results. Detailed preference and emotion breakdowns for \system{} are reported in Appendix~\ref{app:membench-detail}. Bold entries are best; underlined entries are second best.}
\label{tab:reflective}
\centering
\small
\begin{tabular}{@{}l cc@{}}
\toprule
\textbf{Method} & \textbf{10k tokens} & \textbf{100k tokens} \\
\midrule
FullMemory       & 0.733              & 0.533               \\
RecentMemory     & 0.700              & 0.333               \\
RetrievalMemory  & 0.692              & \underline{0.833}   \\
GenerativeAgent  & \underline{0.742}  & 0.333               \\
MemoryBank       & 0.692              & 0.400               \\
MemGPT           & 0.733              & 0.367               \\
SCMemory         & 0.542              & 0.267               \\
\midrule
\system{}        & \textbf{0.843}     & \textbf{0.863}      \\
\bottomrule
\end{tabular}
\end{table}

% \system{} improves from 84.3\% at 10k tokens to 86.3\% at 100k tokens.
% This pattern suggests that incremental extraction into a structured profile can reduce dependence on long raw context at query time.
% As supporting evidence, \system{} reaches Recall@10 of 0.869 at 10k tokens and 0.644 at 100k tokens; its read and write latencies are about 0.04s and 0.06s, respectively.
Table~\ref{tab:reflective} shows that \system{} achieves the highest reflective accuracy at both context lengths.
At 10k tokens, it improves over the strongest prior baseline from 0.742 to 0.843.
At 100k tokens, it improves over the strongest prior baseline from 0.833 to 0.863.
These results suggest that the structured memory backbone can preserve reflective user information over long contexts, providing a reliable substrate for downstream proactive prediction.
As supporting diagnostics, \system{} reaches Recall@10 of 0.869 at 10k tokens and 0.644 at 100k tokens, with read and write latencies of approximately 0.04s and 0.06s, respectively.

% \subsection{ProActEval Main Results}
% \label{sec:exp:proactivebench}

% We evaluate all 200 ProActEval scenarios under three conditions.
% The Reactive condition disables both future-state prediction and idle-time Acquisition.
% Undirected Idle enables idle-time Acquisition without predictive direction, using unguided background intents.
% Directed Idle enables both Future-State Prediction and Idle-Time Acquisition; this is the full \system{} configuration.
% This design separates the value of idle compute from the value of directing that compute toward predicted future needs.


% Directed Idle improves every non-cost metric over both baselines.
% The comparison with Reactive shows the end-to-end value of proactivity.
% The comparison with Undirected Idle shows that background search alone is not sufficient: undirected exploration spends substantial active-token budget but only slightly improves over the reactive baseline.
% In contrast, Directed Idle uses future-state prediction to guide exploration, reducing user effort by 10.7\% and $T_{100}$ by 14.1\% relative to Undirected Idle.

% \subsection{Module Ablation: Direction Matters}

% The ablation isolates the two modules and tests whether direction matters.
% Undirected Idle keeps Idle-Time Acquisition but removes Future-State Prediction.
% It improves $T_{100}$ by only 0.9\% over Reactive and reduces user effort by 1.1\%, despite using 69.8k active tokens per scenario on average.
% Directed Idle adds prediction-guided direction and improves $T_{100}$ by 14.8\% and user effort by 11.7\% over Reactive.
% This gap indicates that the main benefit comes from assigning idle-time compute to needs that are likely to become relevant, not from increasing background search volume by itself.

\subsection{Search Budget Analysis}
\label{sec:exp:budget-scaling}

% We further vary the maximum number of idle-time compute on a matched 50-scenario subset.
% For each budget $k \in \{4,8,12,16\}$, we compare Directed Idle ($k$) against Undirected Idle ($k$).
% This sweep asks whether more idle-time compute monotonically improves end-to-end interaction quality.
% Figure~\ref{fig:budget-scaling} focuses on the matched-budget efficiency and cost endpoints: completion turns, explicit user effort, and active-token usage.

We further study how the amount of idle-time acquisition affects proactive assistance.
On a matched 50-scenario subset, we vary the search budget $k \in \{4,8,12,16\}$ and compare \textsc{Directed Idle}$(k)$ with \textsc{Undirected Idle}$(k)$ under the same budget.
This controlled sweep tests whether increasing idle-time search monotonically improves interaction efficiency, and whether predictive direction remains beneficial when search volume is matched, and whether higher budgets continue to expand anticipation recall.
Figure~\ref{fig:budget-scaling} reports four endpoints: completion turns, explicit user effort, anticipation recall and active-token cost.


\begin{figure*}[t]
\centering
\definecolor{undirblue}{HTML}{4C78A8}
\definecolor{fullred}{HTML}{C44E52}
\definecolor{axisgray}{HTML}{6E6E6E}
\pgfplotsset{
budgetaxis/.style={
    width=\linewidth,
    height=3.25cm,
    xmin=3.2, xmax=16.8,
    xtick={4,8,12,16},
    xlabel={Search budget $k$},
    tick label style={font=\scriptsize},
    label style={font=\scriptsize},
    title style={font=\footnotesize\bfseries, yshift=-0.4ex},
    axis x line*=bottom,
    axis y line*=left,
    axis line style={axisgray!60},
    tick style={axisgray!60},
    ymajorgrids=true,
    grid style={gray!16},
    minor tick num=0,
}}
\begin{tikzpicture}[baseline]
    \draw[undirblue, line width=0.8pt] (0,0) circle (1.8pt);
    \node[anchor=west, font=\scriptsize] at (0.13,0) {Undirected};
    \filldraw[fullred] (1.72,0) circle (1.9pt);
    \node[anchor=west, font=\scriptsize] at (1.85,0) {Directed};
    \draw[gray!50, line width=1.2pt] (3.20,-0.10) -- (3.20,0.10);
    \node[anchor=west, font=\scriptsize] at (3.34,0) {matched-budget gap};
\end{tikzpicture}

\vspace{0.35em}

\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    budgetaxis,
    title={(a) Faster completion},
    ylabel={$T_{100}$},
    ymin=6.2, ymax=8.4,
    ytick={6.5,7.0,7.5,8.0},
]
\draw[gray!45, line width=1.15pt] (axis cs:4,6.56) -- (axis cs:4,8.10);
\draw[gray!45, line width=1.15pt] (axis cs:8,6.64) -- (axis cs:8,7.70);
\draw[gray!45, line width=1.15pt] (axis cs:12,6.80) -- (axis cs:12,7.74);
\draw[gray!45, line width=1.15pt] (axis cs:16,6.62) -- (axis cs:16,7.52);
\addplot+[only marks, mark=o, mark size=2.1pt, draw=undirblue, fill=white, line width=0.9pt]
    coordinates {(4,8.10) (8,7.70) (12,7.74) (16,7.52)};
\addplot+[only marks, mark=*, mark size=2.2pt, draw=fullred, fill=fullred]
    coordinates {(4,6.56) (8,6.64) (12,6.80) (16,6.62)};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    budgetaxis,
    title={(b) Fewer explicit turns},
    ylabel={User Effort},
    ymin=7.5, ymax=9.3,
    ytick={7.5,8.0,8.5,9.0},
]
\draw[gray!45, line width=1.15pt] (axis cs:4,8.02) -- (axis cs:4,9.00);
\draw[gray!45, line width=1.15pt] (axis cs:8,7.90) -- (axis cs:8,8.84);
\draw[gray!45, line width=1.15pt] (axis cs:12,8.18) -- (axis cs:12,8.78);
\draw[gray!45, line width=1.15pt] (axis cs:16,7.82) -- (axis cs:16,8.62);
\addplot+[only marks, mark=o, mark size=2.1pt, draw=undirblue, fill=white, line width=0.9pt]
    coordinates {(4,9.00) (8,8.84) (12,8.78) (16,8.62)};
\addplot+[only marks, mark=*, mark size=2.2pt, draw=fullred, fill=fullred]
    coordinates {(4,8.02) (8,7.90) (12,8.18) (16,7.82)};
\end{axis}
\end{tikzpicture}
\end{subfigure}

\par\vspace{0.45em}

\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    budgetaxis,
    title={(c) Anticipation recall},
    ylabel={Ant. Recall},
    ymin=-0.03, ymax=0.48,
    ytick={0,0.1,0.2,0.3,0.4},
]
\draw[gray!45, line width=1.15pt] (axis cs:4,0.000) -- (axis cs:4,0.253);
\draw[gray!45, line width=1.15pt] (axis cs:8,0.000) -- (axis cs:8,0.348);
\draw[gray!45, line width=1.15pt] (axis cs:12,0.000) -- (axis cs:12,0.373);
\draw[gray!45, line width=1.15pt] (axis cs:16,0.000) -- (axis cs:16,0.432);
\addplot+[only marks, mark=o, mark size=2.1pt, draw=undirblue, fill=white, line width=0.9pt]
    coordinates {(4,0.000) (8,0.000) (12,0.000) (16,0.000)};
\addplot+[only marks, mark=*, mark size=2.2pt, draw=fullred, fill=fullred]
    coordinates {(4,0.253) (8,0.348) (12,0.373) (16,0.432)};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.485\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
    budgetaxis,
    title={(d) Active-token cost},
    ylabel={Active Tokens (k)},
    ymin=0, ymax=125,
    ytick={0,25,50,75,100},
    ybar,
    bar width=4.5pt,
    enlarge x limits=0.12,
]
\addplot+[draw=undirblue, fill=undirblue!28, bar shift=-3pt]
    coordinates {(4,11.3) (8,23.4) (12,35.5) (16,48.6)};
\addplot+[draw=fullred, fill=fullred!70, bar shift=3pt]
    coordinates {(4,62.5) (8,75.8) (12,89.8) (16,97.0)};
\node[font=\tiny, text=fullred, anchor=south] at (axis cs:4,65.0) {+51k};
\node[font=\tiny, text=fullred, anchor=south] at (axis cs:8,78.3) {+52k};
\node[font=\tiny, text=fullred, anchor=south] at (axis cs:12,92.3) {+54k};
\node[font=\tiny, text=fullred, anchor=south] at (axis cs:16,99.5) {+48k};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Effect of search budget on a matched 50-scenario subset. Panels (a)--(c) use paired gaps: gray segments connect Undirected Idle ($k$) and Directed Idle ($k$) under the same search budget. Panel (c) shows that increasing budget raises Directed Idle anticipation recall, while Undirected Idle remains at zero. Panel (d) reports active-token cost in thousands; labels above Directed Idle bars show additional cost relative to Undirected Idle. Prediction-guided exploration yields smaller $T_{100}$ and fewer explicit user turns at every budget, but the efficiency gains flatten and fluctuate as $k$ increases.}
\label{fig:budget-scaling}
\end{figure*}

% The budget experiment shows a cost--efficiency trade-off, not a simple ``more search is always better'' pattern.
% At every matched budget, Directed Idle achieves smaller $T_{100}$ and fewer explicit user turns than Undirected Idle, showing that predictive direction matters beyond search volume alone.
% However, the gains are non-monotonic: increasing $k$ raises active-token cost steadily, while $T_{100}$ and user effort flatten or fluctuate.
% The reason is that each budget is an independent closed-loop run: additional searches can change memory contents, push timing, and later dialogue context.
% Thus, search budget should be treated as an operating-point choice rather than a knob to maximize.

Figure~\ref{fig:budget-scaling} shows a clear cost--efficiency trade-off rather than a simple ``more search is better'' trend.
At every matched budget, \textsc{Directed Idle} achieves lower $T_{100}$ and lower User Effort than \textsc{Undirected Idle}, indicating that predictive direction improves the utility of idle-time acquisition beyond search volume alone.
Increasing $k$ continues to raise \textsc{Directed Idle}'s Anticipation Recall, from 0.253 at $k=4$ to 0.432 at $k=16$, but under the finite-scenario setting of ProActEval that extra recall does not guarantee monotonic reductions in User Effort.
Once the main predictable needs are covered, additional searches tend to chase lower-marginal or later needs, and each budget setting also induces a different closed-loop trajectory by changing memory contents, push timing, and subsequent dialogue context.
As a result, active-token cost rises steadily while $T_{100}$ and User Effort flatten or fluctuate.
Thus, the search budget should be treated as an operating point that balances efficiency gains against compute cost, rather than as a parameter to maximize.

\subsection{Discussion}
\label{sec:exp:discussion}

The experiments support three conclusions.
First, MemBench shows that \system{}'s memory layer is strong enough to support long-horizon personalization.
Second, ProActEval shows that Future-State Prediction combined with directed Idle-Time Acquisition improves end-to-end performance across efficiency, coverage, and factual-integrity metrics.
Third, the comparison with ProactiveAgent-style prompting suggests that frequent proactive attempts are not sufficient by themselves: a system can produce many \texttt{Proactive\_Task} outputs while still rarely covering benchmark-labeled predictable needs.

At the same time, the ProactiveAgent comparison highlights an important limitation of the current design and evaluation.
\system{} achieves much higher judge-labeled Anticipation Recall than ProactiveAgent-style prompting, but the corresponding gains in $T_{100}$ and User Effort are more modest.
This indicates that anticipating predictable needs does not translate linearly into fewer dialogue turns.
End-to-end efficiency can still be bottlenecked by the last few uncovered needs, by simulator continuation policies, and by strong full-context reactive baselines that can answer accurately once the user asks.
Future work should therefore optimize not only which predicted needs are prepared, but also when and how proactive delivery changes the subsequent dialogue trajectory.

% The experiments support three conclusions.
% MemBench shows that \system{}'s memory layer is strong enough to support long-horizon personalization.
% ProActEval shows that proactive prediction combined with directed idle-time Acquisition improves end-to-end performance across efficiency, coverage, and factual-integrity metrics.
% The budget results also show that idle-time compute has a real cost.
% The best operating point should therefore be chosen by balancing efficiency gains, hallucination risk, and active-token budget.


==> sections/method.tex <==
% ====================================================================
% Section 3: Method
% ====================================================================

\section{Method}
\label{sec:method}

\subsection{Overview}
\label{sec:method:overview}

\system{} is designed for multi-turn proactive search.
Given an ongoing interaction, the assistant should infer what the user is likely to need next, prepare relevant information during idle periods, and surface it only when the expected benefit outweighs the cost of interruption.
As shown in Figure~\ref{fig:architecture}, \system{} builds proactive search around an Idle-Time compute mechanism grounded in persistent memory and regulated by a utility-aware delivery policy.
This mechanism is driven by two core modules.
\textbf{Future-State Prediction} estimates likely upcoming user needs from the current dialogue history and memory state, while \textbf{Idle-Time Acquisition} allocates background computation to high-value candidates through evidence retrieval and synthesis.
A personalized memory layer provides the state that grounds prediction, exposes knowledge gaps, and stores newly acquired evidence.


\begin{figure}[!t]
  \centering
  \safeincludegraphics[width=\linewidth]{figures/overview.drawio.png}
  \vspace{-1.5em}
  \caption{\system{} overview. The assistant updates a persistent memory state after each foreground interaction, predicts likely upcoming user needs during idle intervals, and acquires supporting evidence for high-value candidates. A utility-aware delivery policy decides whether the prepared content should be proactively delivered, woven into a subsequent response, or silently stored for future use.}
  \label{fig:architecture}
\end{figure}

\subsection{Problem Formulation and Design Objectives}
\label{sec:method:formulation}

At turn $t$, the assistant observes the dialogue history $H_t$ and a persistent memory state $M_t$.
The memory state $M_t$ summarizes information accumulated before turn $t$, including
user profile attributes, entity-level facts, conversation summaries, and
previously acquired research artifacts.
After answering the current user request, the system may receive an idle window $\Delta_t$ with search budget $B_t$.
We denote the overall proactive policy by $\pi$: it chooses candidate future needs $z \in \mathcal{Z}_t$, allocates budget to a subset of them, and selects a delivery action $d_z \in \{\mathrm{push}, \mathrm{queue}, \mathrm{store}\}$ for any resulting artifact.
Its objective is not to maximize search volume, but to improve future task progress while controlling interruption, cost, and factual risk:
\[
\max_{\pi}\; \mathbb{E}\big[
U_{\text{future}}(\pi; H_t,M_t)
- \lambda_i C_{\text{interrupt}}(\pi)
- \lambda_b C_{\text{budget}}(\pi)
- \lambda_h R_{\text{hallucination}}(\pi)
\big].
\]
We use this objective as a design guide rather than a directly optimized training loss.
The objective leads to three design requirements.
Candidates should correspond to needs likely to arise later, proactive artifacts should be supported by remembered or retrieved evidence, and useful information should be pushed only when its expected value exceeds the cost of distracting the user.
Future-State Prediction estimates $\mathcal{Z}_t$ from $(H_t,M_t)$, Idle-Time Acquisition searches the high-value subset under budget, and successful exploration updates $M_{t+1}$ so later predictions can use both interaction history and previously prepared evidence.

\subsection{Future-State Prediction Module}
\label{sec:method:fsp}

Proactive assistance depends on a form of prospective memory: the system must recognize that a current user state implies likely future needs.
In multi-turn conversations, these needs are not isolated labels.
They emerge from the user's current activity, prior interests, partially satisfied goals, and knowledge gaps that remain unresolved after previous turns.
The purpose of Future-State Prediction is therefore to estimate a compact candidate set $\mathcal{Z}_t$ before the user explicitly asks for those needs.

Each predicted need is represented as a structured candidate rather than a
free-form sentence. In our implementation, a candidate contains a topic, a
natural-language need description, a reason grounded in the recent dialogue or
memory state, a confidence estimate, and a retrieval query. The confidence
estimate is used for filtering, the topic field supports deduplication, and the
retrieval query is passed to the acquisition module.

\paragraph{Candidate generation.}
The predictor generates candidate needs from two complementary sources.
It uses local scenario prediction to extrapolate likely next-step needs from the recent dialogue and the user's immediate task.
It also uses related expansion, which proposes adjacent topics grounded in persistent profile and conversation memory.
Local prediction targets near-term follow-up questions, while related expansion broadens the frontier of useful support during longer idle gaps.

\paragraph{Memory-gap augmentation.}
The predictor also receives signals from memory maintenance.
When the memory layer identifies stale, incomplete, or weakly supported knowledge, those gaps become candidate directions for future exploration.
This design makes memory active: it does not only store prior context, but also proposes missing information that may become useful in later turns.

\paragraph{Filtering and prioritization.}
Predicted needs are filtered by confidence and deduplicated against recent research history.
The remaining candidates enter a priority queue keyed by normalized topic similarity.
This keeps the prediction stage conservative enough to avoid repeatedly exploring near-duplicate topics while still preserving multiple plausible future directions.

\subsection{Idle-Time Acquisition Module}
\label{sec:method:ite}

Predicting a possible future need is not sufficient.
Idle computing is finite, and not every plausible topic deserves search, synthesis, or user-facing delivery.
The Idle-Time Acquisition module realizes the budgeted allocation part of the formulation: spend background compute where it is likely to reduce future user effort, improve coverage, or improve factual grounding.

\paragraph{Value evaluation.}
Each candidate is scored along four dimensions: user relevance $(r)$, knowledge gap $(g)$, incremental value $(v)$, and timeliness $(t)$.
The module computes
\[
S = w_r r + w_g g + w_v v + w_t t, \qquad \sum_i w_i = 1,
\]
where user relevance $(r)$ measures whether the candidate follows from the current task or stable user profile, and knowledge gap $(g)$ measures whether existing memory lacks sufficient evidence for the candidate.
Incremental value $(v)$ measures whether acquiring the information would add non-redundant support beyond stored memory, while timeliness $(t)$ measures whether the information is likely to be useful before the next user turn or a near-term topic shift.
    

The module does not immediately acquire candidates below a value threshold $\theta_{\text{val}}$.

This gate prevents Idle-Time compute from degenerating into unconditional background retrieval.
It also operationalizes interruption control: low-value candidates may remain in memory or the queue, but they are not allowed to consume immediate search and delivery budget.

\paragraph{Iterative exploration.}
Accepted candidates are decomposed into subtopics and explored through repeated search, evidence extraction, and coverage checking.
Before launching new search, the module checks whether existing memory already covers the topic.
If prior coverage is sufficient, the system reuses memory; if coverage is partial, it searches only for the missing subtopics.
This makes idle-time compute incremental rather than a full restart on every predicted need.

\paragraph{Synthesis and delivery.}
Retrieved evidence is synthesized into a compact knowledge artifact with provenance.
The provenance records the remembered or retrieved evidence used to support the synthesized artifact.
A delivery policy then decides whether the artifact should be pushed immediately, queued for later use, or stored silently.
The policy balances expected value against interruption cost.
This final gate is essential because proactive systems can harm the interaction if they surface low-value information at the wrong time.

\subsection{Memory Support}
\label{sec:method:memory}

\system{} uses personalized memory as the state variable $M_t$ in the proactive loop.
The memory layer stores user profiles, entity-level facts, conversation summaries, and research knowledge.
Within the proactive loop, memory is used in three ways.
It provides profile and dialogue evidence for Future-State Prediction, is queried
before Idle-Time Acquisition to check whether a candidate need is already
covered, and stores synthesized artifacts with provenance for later reuse.
It supports semantic and temporal retrieval for downstream modules, and it is updated after user--assistant turns as well as after successful idle-time Acquisition.
This makes memory a grounding substrate rather than the main objective of the system: memory conditions the next prediction, and proactive exploration improves the evidence available to future turns.


==> sections/old_references.tex <==
\begin{thebibliography}{14}
\small

\bibitem[Park et~al.(2023)]{generativeagent}
Park, J.~S., O'Brien, J.~C., Cai, C.~J., Morris, M.~R., Liang, P., and Bernstein, M.~S.
Generative agents: Interactive simulacra of human behavior.
In \emph{UIST}, 2023.

\bibitem[Packer et~al.(2023)]{memgpt}
Packer, C., Wooders, S., Lin, K., Fang, V., Patil, S.~G., Stoica, I., and Gonzalez, J.~E.
MemGPT: Towards LLMs as operating systems.
\emph{arXiv preprint arXiv:2310.08560}, 2023.

\bibitem[Zhong et~al.(2024)]{memorybank}
Zhong, W., Guo, L., Gao, Q., and Wang, Y.
MemoryBank: Enhancing large language models with long-term memory.
In \emph{AAAI}, 2024.


\bibitem[Wang et~al.(2023)]{scmemory}
Wang, B., Liang, X., Yang, J., Huang, H., Wu, S., Wu, P., Lu, L., Ma, Z., and Li, Z.
Enhancing large language model with self-controlled memory framework.
\emph{arXiv preprint arXiv:2304.13343}, 2023.

\bibitem[Tennenholtz et~al.(2023)]{proactivecomputing}
Tennenholtz, G., Hick, R., and Mannor, S.
Proactive computing: Foundations and implementations.
\emph{ACM Computing Surveys}, 2023.

\bibitem[Deng et~al.(2023)]{proactivedialog}
Deng, Y., Zhang, W., Chen, Z., and Gu, Q.
Proactive dialogue systems: A survey.
\emph{arXiv preprint arXiv:2305.02750}, 2023.

\bibitem[Shinn et~al.(2023)]{reflexion}
Shinn, N., Cassano, F., Gopinath, A., Narasimhan, K., and Yao, S.
Reflexion: Language agents with verbal reinforcement learning.
In \emph{NeurIPS}, 2023.

\bibitem[Su et~al.(2019)]{collaborative}
Su, Y., Yang, D., Ostendorf, M., and Hovy, E.
Collaborative filtering for conversational recommendation.
In \emph{ACL}, 2019.

\bibitem[Salemi et~al.(2024)]{personallm}
Salemi, A., Mysore, S., Bendersky, M., and Zamani, H.
LaMP: When large language models meet personalization.
In \emph{NAACL}, 2024.

\bibitem[Tan et~al.(2025)]{membench}
Tan, H., Zhang, Z., Ma, C., Chen, X., Dai, Q., and Dong, Z.
MemBench: Towards More Comprehensive Evaluation on the Memory of LLM-based Agents.
In \emph{Findings of the Association for Computational Linguistics: ACL 2025}, pages 19336--19352, 2025.
doi:10.18653/v1/2025.findings-acl.989.

\bibitem[Wu et~al.(2024)]{longmemeval}
Wu, Y., Xie, T., Jiao, W., Ye, Z., Chen, J., Li, T., and Wen, Z.
LongMemEval: Benchmarking chat assistants on long-term interactive memory.
\emph{arXiv preprint arXiv:2410.10813}, 2024.

\bibitem[Zhang et~al.(2024)]{memsim}
Zhang, Z., Bo, L., Xiao, C., Chen, H., and Chen, H.
MemSim: A Bayesian simulator for evaluating memory of LLM-based personal assistants.
\emph{arXiv preprint arXiv:2409.20163}, 2024.

\bibitem[Du et~al.(2024)]{perltqa}
Du, Z., Chen, Q., Jia, Y., Chen, X., Xie, R., Ji, Z., and Sun, M.
PerLTQA: A personal long-term memory dataset for memory classification, retrieval, and synthesis in question answering.
\emph{arXiv preprint arXiv:2402.16288}, 2024.

\bibitem[Kim et~al.(2024)]{dialsim}
Kim, J., Lee, J., Yoo, K.~M., and Kang, J.
DialSim: A real-time simulator for evaluating long-term dialogue understanding of conversational agents.
\emph{arXiv preprint arXiv:2406.13144}, 2024.

\end{thebibliography}


==> sections/proactivebench_design.tex <==
\subsubsection{Benchmark Design}

To evaluate proactive assistance, we construct \textsc{ProactiveBench}, a benchmark designed to measure whether an assistant can anticipate user information needs before they are explicitly asked. Existing memory benchmarks mainly assess recall and reasoning over stored context, but they do not directly test proactive anticipation. Our benchmark addresses this gap by modeling users in unfamiliar but realistic situations, where resolving earlier questions can make later needs reasonably predictable. To keep the evaluation controlled, all scenarios are grounded in closed-world fact sheets rather than open-ended world knowledge.

\paragraph{Scenario structure.}
Each \textsc{ProactiveBench} instance is a fact-grounded conversational scenario. A scenario contains a user profile, a fact sheet, and an ordered sequence of user needs. The user profile specifies the persona, current situation, and communication style. The fact sheet provides scenario-specific ground truth as atomic, verifiable facts. The user needs represent the information needs that may arise during the conversation; each need is annotated with an importance label (must-have or nice-to-have), one or more \texttt{key\_fact\_ids} that directly ground the need, and a \texttt{predictable\_after} relation indicating when the need becomes reasonably anticipatable after an earlier one has been addressed. This structure allows us to distinguish reactive responses to explicit questions from proactive delivery of future-relevant information.

\paragraph{Data generation pipeline.}
We synthesize the benchmark through a staged generation pipeline. Starting from manually designed seed scenarios, we first generate scenario-specific fact sheets and then generate user needs conditioned on those facts. To avoid contamination from parametric world knowledge, core entities such as organizations, people, addresses, emails, and internal URLs are required to be fictional, while generic tools and standards may retain real names when appropriate. Generated scenarios then undergo multi-level quality control. Automatic validation checks structural consistency, including identifier uniqueness, validity of fact grounding, legal and acyclic predictability links, turn ordering, and reveal-group consistency. For grouped scenarios, we additionally require sufficient cross-group predictability and auditable proactive targets so that the benchmark preserves measurable headroom for proactive behavior. Beyond structural checks, scenarios are manually reviewed for factual consistency, realism of need progression, strength of predictability links, and judge-friendliness, ensuring that proactive targets are both plausible and cleanly evaluable.
\textsc{ProactiveBench} currently includes validated scenarios spanning multiple domains, with each scenario designed to support evaluation of proactive anticipation, user-effort reduction, and factual integrity under a unified protocol. We summarize the final benchmark statistics below.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{sections/proactivebench_stats_figure.pdf}
    \caption{
    Composition statistics of ProactiveBench.
    Panel (a) shows the distribution of user-need counts across scenarios.
    Panel (b) shows the distribution of fact-sheet sizes across scenarios.
    Panel (c) summarizes the benchmark's breadth across coarse-grained application categories, demonstrating that ProactiveBench spans diverse real-world settings rather than concentrating on a narrow task family.
    Panel (d) reports benchmark-wide counts of predictable versus non-predictable needs, cross-group versus intra-group prediction links, and auditable proactive targets.
    Together, these statistics show that ProactiveBench combines broad domain coverage, structured multi-need scenarios, and substantial measurable headroom for evaluating proactive assistance.}
    \label{fig:proactivebench_composition}
\end{figure*}

